Search for the leptonic decay $D^{+}\to e^{+}\nu_{e}$

We search for the leptonic decay $D^+\to e^+\nu_{e}$ using an $e^+e^-$ collision data sample with an integrated luminosity of 20.3~fb$^{-1}$ collected with the BESIII detector at the center-of-mass energy of 3.773~GeV. No significant signal is observed and an upper limit on the branching fraction of $D^+\to e^+\nu_{e}$ is set as $9.7 \times 10^{-7}$, at the 90\% confidence level. Our upper limit is an order of magnitude smaller than the previous limit for this decay mode.

==> Source/authorlist_2024-04-24_Chinese.tex <==
%\author{Author list}
%\begin{small}
%\begin{center}
\author{
\small
  M.~Ablikim(麦迪娜)$^{1}$, M.~N.~Achasov$^{4,c}$, P.~Adlarson$^{76}$, O.~Afedulidis$^{3}$, X.~C.~Ai(艾小聪)$^{81}$, R.~Aliberti$^{35}$, A.~Amoroso$^{75A,75C}$, Q.~An(安琪)$^{72,58,a}$, Y.~Bai(白羽)$^{57}$, O.~Bakina$^{36}$, I.~Balossino$^{29A}$, Y.~Ban(班勇)$^{46,h}$, H.-R.~Bao(包浩然)$^{64}$, V.~Batozskaya$^{1,44}$, K.~Begzsuren$^{32}$, N.~Berger$^{35}$, M.~Berlowski$^{44}$, M.~Bertani$^{28A}$, D.~Bettoni$^{29A}$, F.~Bianchi$^{75A,75C}$, E.~Bianco$^{75A,75C}$, A.~Bortone$^{75A,75C}$, I.~Boyko$^{36}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{69}$, H.~Cai(蔡浩)$^{77}$, X.~Cai(蔡啸)$^{1,58}$, A.~Calcaterra$^{28A}$, G.~F.~Cao(曹国富)$^{1,64}$, N.~Cao(曹宁)$^{1,64}$, S.~A.~Cetin$^{62A}$, X.~Y.~Chai(柴新宇)$^{46,h}$, J.~F.~Chang(常劲帆)$^{1,58}$, G.~R.~Che(车国荣)$^{43}$, Y.~Z.~Che(车逾之)$^{1,58,64}$, G.~Chelkov$^{36,b}$, C.~Chen(陈琛)$^{43}$, C.~H.~Chen(陈春卉)$^{9}$, Chao~Chen(陈超)$^{55}$, G.~Chen(陈刚)$^{1}$, H.~S.~Chen(陈和生)$^{1,64}$, H.~Y.~Chen(陈弘扬)$^{20}$, M.~L.~Chen(陈玛丽)$^{1,58,64}$, S.~J.~Chen(陈申见)$^{42}$, S.~L.~Chen(陈思璐)$^{45}$, S.~M.~Chen(陈少敏)$^{61}$, T.~Chen(陈通)$^{1,64}$, X.~R.~Chen(陈旭荣)$^{31,64}$, X.~T.~Chen(陈肖婷)$^{1,64}$, Y.~B.~Chen(陈元柏)$^{1,58}$, Y.~Q.~Chen$^{34}$, Z.~J.~Chen(陈卓俊)$^{25,i}$, Z.~Y.~Chen(陈正元)$^{1,64}$, S.~K.~Choi$^{10}$, G.~Cibinetto$^{29A}$, F.~Cossio$^{75C}$, J.~J.~Cui(崔佳佳)$^{50}$, H.~L.~Dai(代洪亮)$^{1,58}$, J.~P.~Dai(代建平)$^{79}$, A.~Dbeyssi$^{18}$, R.~ E.~de Boer$^{3}$, D.~Dedovich$^{36}$, C.~Q.~Deng(邓创旗)$^{73}$, Z.~Y.~Deng(邓子艳)$^{1}$, A.~Denig$^{35}$, I.~Denysenko$^{36}$, M.~Destefanis$^{75A,75C}$, F.~De~Mori$^{75A,75C}$, B.~Ding(丁彪)$^{67,1}$, X.~X.~Ding(丁晓萱)$^{46,h}$, Y.~Ding(丁勇)$^{40}$, Y.~Ding(丁逸)$^{34}$, J.~Dong(董静)$^{1,58}$, L.~Y.~Dong(董燎原)$^{1,64}$, M.~Y.~Dong(董明义)$^{1,58,64}$, X.~Dong(董翔)$^{77}$, M.~C.~Du(杜蒙川)$^{1}$, S.~X.~Du(杜书先)$^{81}$, Y.~Y.~Duan(段尧予)$^{55}$, Z.~H.~Duan(段宗欢)$^{42}$, P.~Egorov$^{36,b}$, Y.~H.~Fan(范宇晗)$^{45}$, J.~Fang(方建)$^{1,58}$, J.~Fang(方进)$^{59}$, S.~S.~Fang(房双世)$^{1,64}$, W.~X.~Fang(方文兴)$^{1}$, Y.~Fang(方易)$^{1}$, Y.~Q.~Fang(方亚泉)$^{1,58}$, R.~Farinelli$^{29A}$, L.~Fava$^{75B,75C}$, F.~Feldbauer$^{3}$, G.~Felici$^{28A}$, C.~Q.~Feng(封常青)$^{72,58}$, J.~H.~Feng(冯俊华)$^{59}$, Y.~T.~Feng(冯玙潼)$^{72,58}$, M.~Fritsch$^{3}$, C.~D.~Fu(傅成栋)$^{1}$, J.~L.~Fu(傅金林)$^{64}$, Y.~W.~Fu(傅亦威)$^{1,64}$, H.~Gao(高涵)$^{64}$, X.~B.~Gao(高鑫博)$^{41}$, Y.~N.~Gao(高原宁)$^{46,h}$, Yang~Gao(高扬)$^{72,58}$, S.~Garbolino$^{75C}$, I.~Garzia$^{29A,29B}$, L.~Ge(葛玲)$^{81}$, P.~T.~Ge(葛潘婷)$^{19}$, Z.~W.~Ge(葛振武)$^{42}$, C.~Geng(耿聪)$^{59}$, E.~M.~Gersabeck$^{68}$, A.~Gilman$^{70}$, K.~Goetzen$^{13}$, L.~Gong(龚丽)$^{40}$, W.~X.~Gong(龚文煊)$^{1,58}$, W.~Gradl$^{35}$, S.~Gramigna$^{29A,29B}$, M.~Greco$^{75A,75C}$, M.~H.~Gu(顾旻皓)$^{1,58}$, Y.~T.~Gu(顾运厅)$^{15}$, C.~Y.~Guan(关春懿)$^{1,64}$, A.~Q.~Guo(郭爱强)$^{31,64}$, L.~B.~Guo(郭立波)$^{41}$, M.~J.~Guo(国梦娇)$^{50}$, R.~P.~Guo(郭如盼)$^{49}$, Y.~P.~Guo(郭玉萍)$^{12,g}$, A.~Guskov$^{36,b}$, J.~Gutierrez$^{27}$, K.~L.~Han(韩坤霖)$^{64}$, T.~T.~Han(韩婷婷)$^{1}$, F.~Hanisch$^{3}$, X.~Q.~Hao(郝喜庆)$^{19}$, F.~A.~Harris$^{66}$, K.~K.~He(何凯凯)$^{55}$, K.~L.~He(何康林)$^{1,64}$, F.~H.~Heinsius$^{3}$, C.~H.~Heinz$^{35}$, Y.~K.~Heng(衡月昆)$^{1,58,64}$, C.~Herold$^{60}$, T.~Holtmann$^{3}$, P.~C.~Hong(洪鹏程)$^{34}$, G.~Y.~Hou(侯国一)$^{1,64}$, X.~T.~Hou(侯贤涛)$^{1,64}$, Y.~R.~Hou(侯颖锐)$^{64}$, Z.~L.~Hou(侯治龙)$^{1}$, B.~Y.~Hu(胡碧颖)$^{59}$, H.~M.~Hu(胡海明)$^{1,64}$, J.~F.~Hu(胡继峰)$^{56,j}$, S.~L.~Hu(胡圣亮)$^{12,g}$, T.~Hu(胡涛)$^{1,58,64}$, Y.~Hu(胡誉)$^{1}$, G.~S.~Huang(黄光顺)$^{72,58}$, K.~X.~Huang(黄凯旋)$^{59}$, L.~Q.~Huang(黄麟钦)$^{31,64}$, X.~T.~Huang(黄性涛)$^{50}$, Y.~P.~Huang(黄燕萍)$^{1}$, Y.~S.~Huang(黄永盛)$^{59}$, T.~Hussain$^{74}$, F.~H\"olzken$^{3}$, N.~H\"usken$^{35}$, N.~in der Wiesche$^{69}$, J.~Jackson$^{27}$, S.~Janchiv$^{32}$, J.~H.~Jeong$^{10}$, Q.~Ji(纪全)$^{1}$, Q.~P.~Ji(姬清平)$^{19}$, W.~Ji(季旺)$^{1,64}$, X.~B.~Ji(季晓斌)$^{1,64}$, X.~L.~Ji(季筱璐)$^{1,58}$, Y.~Y.~Ji(吉钰瑶)$^{50}$, X.~Q.~Jia(贾晓倩)$^{50}$, Z.~K.~Jia(贾泽坤)$^{72,58}$, D.~Jiang(姜地)$^{1,64}$, H.~B.~Jiang(姜候兵)$^{77}$, P.~C.~Jiang(蒋沛成)$^{46,h}$, S.~S.~Jiang(姜赛赛)$^{39}$, T.~J.~Jiang(蒋庭俊)$^{16}$, X.~S.~Jiang(江晓山)$^{1,58,64}$, Y.~Jiang(蒋艺)$^{64}$, J.~B.~Jiao(焦健斌)$^{50}$, J.~K.~Jiao(焦俊坤)$^{34}$, Z.~Jiao(焦铮)$^{23}$, S.~Jin(金山)$^{42}$, Y.~Jin(金毅)$^{67}$, M.~Q.~Jing(荆茂强)$^{1,64}$, X.~M.~Jing(景新媚)$^{64}$, T.~Johansson$^{76}$, S.~Kabana$^{33}$, N.~Kalantar-Nayestanaki$^{65}$, X.~L.~Kang(康晓琳)$^{9}$, X.~S.~Kang(康晓珅)$^{40}$, M.~Kavatsyuk$^{65}$, B.~C.~Ke(柯百谦)$^{81}$, V.~Khachatryan$^{27}$, A.~Khoukaz$^{69}$, R.~Kiuchi$^{1}$, O.~B.~Kolcu$^{62A}$, B.~Kopf$^{3}$, M.~Kuessner$^{3}$, X.~Kui(奎贤)$^{1,64}$, N.~~Kumar$^{26}$, A.~Kupsc$^{44,76}$, W.~K\"uhn$^{37}$, J.~J.~Lane$^{68}$, L.~Lavezzi$^{75A,75C}$, T.~T.~Lei(雷天天)$^{72,58}$, Z.~H.~Lei(雷祚弘)$^{72,58}$, M.~Lellmann$^{35}$, T.~Lenz$^{35}$, C.~Li(李聪)$^{43}$, C.~Li(李翠)$^{47}$, C.~H.~Li(李春花)$^{39}$, Cheng~Li(李澄)$^{72,58}$, D.~M.~Li(李德民)$^{81}$, F.~Li(李飞)$^{1,58}$, G.~Li(李刚)$^{1}$, H.~B.~Li(李海波)$^{1,64}$, H.~J.~Li(李惠静)$^{19}$, H.~N.~Li(李衡讷)$^{56,j}$, Hui~Li(李慧)$^{43}$, J.~R.~Li(李嘉荣)$^{61}$, J.~S.~Li(李静舒)$^{59}$, K.~Li(李科)$^{1}$, K.~L.~Li(李凯璐)$^{19}$, L.~J.~Li(李林健)$^{1,64}$, L.~K.~Li(李龙科)$^{1}$, Lei~Li(李蕾)$^{48}$, M.~H.~Li(李明浩)$^{43}$, P.~R.~Li(李培荣)$^{38,k,l}$, Q.~M.~Li(李启铭)$^{1,64}$, Q.~X.~Li(李起鑫)$^{50}$, R.~Li( 李燃)$^{17,31}$, S.~X.~Li(李素娴)$^{12}$, T. ~Li(李腾)$^{50}$, W.~D.~Li(李卫东)$^{1,64}$, W.~G.~Li(李卫国)$^{1,a}$, X.~Li(李旭)$^{1,64}$, X.~H.~Li(李旭红)$^{72,58}$, X.~L.~Li(李晓玲)$^{50}$, X.~Y.~Li(李晓宇)$^{1,64}$, X.~Z.~Li(李绪泽)$^{59}$, Y.~G.~Li(李彦谷)$^{46,h}$, Z.~J.~Li(李志军)$^{59}$, Z.~Y.~Li(李紫阳)$^{79}$, C.~Liang(梁畅)$^{42}$, H.~Liang(梁浩)$^{1,64}$, H.~Liang(梁昊)$^{72,58}$, Y.~F.~Liang(梁勇飞)$^{54}$, Y.~T.~Liang(梁羽铁)$^{31,64}$, G.~R.~Liao(廖广睿)$^{14}$, Y.~P.~Liao(廖一朴)$^{1,64}$, J.~Libby$^{26}$, A. ~Limphirat$^{60}$, C.~C.~Lin(蔺长城)$^{55}$, D.~X.~Lin(林德旭)$^{31,64}$, T.~Lin(林韬)$^{1}$, B.~J.~Liu(刘北江)$^{1}$, B.~X.~Liu(刘宝鑫)$^{77}$, C.~Liu(刘成)$^{34}$, C.~X.~Liu(刘春秀)$^{1}$, F.~Liu(刘芳)$^{1}$, F.~H.~Liu(刘福虎)$^{53}$, Feng~Liu(刘峰)$^{6}$, G.~M.~Liu(刘国明)$^{56,j}$, H.~Liu(刘昊)$^{38,k,l}$, H.~B.~Liu(刘宏邦)$^{15}$, H.~H.~Liu(刘欢欢)$^{1}$, H.~M.~Liu(刘怀民)$^{1,64}$, Huihui~Liu(刘汇慧)$^{21}$, J.~B.~Liu(刘建北)$^{72,58}$, J.~Y.~Liu(刘晶译)$^{1,64}$, K.~Liu(刘凯)$^{38,k,l}$, K.~Y.~Liu(刘魁勇)$^{40}$, Ke~Liu(刘珂)$^{22}$, L.~Liu(刘亮)$^{72,58}$, L.~C.~Liu(刘良辰)$^{43}$, Lu~Liu(刘露)$^{43}$, M.~H.~Liu(刘美宏)$^{12,g}$, P.~L.~Liu(刘佩莲)$^{1}$, Q.~Liu(刘倩)$^{64}$, S.~B.~Liu(刘树彬)$^{72,58}$, T.~Liu(刘桐)$^{12,g}$, W.~K.~Liu(刘维克)$^{43}$, W.~M.~Liu(刘卫民)$^{72,58}$, X.~Liu(刘翔)$^{38,k,l}$, X.~Liu(刘鑫)$^{39}$, Y.~Liu(刘义)$^{81}$, Y.~Liu(刘英)$^{38,k,l}$, Y.~B.~Liu(刘玉斌)$^{43}$, Z.~A.~Liu(刘振安)$^{1,58,64}$, Z.~D.~Liu(刘宗德)$^{9}$, Z.~Q.~Liu(刘智青)$^{50}$, X.~C.~Lou(娄辛丑)$^{1,58,64}$, F.~X.~Lu(卢飞翔)$^{59}$, H.~J.~Lu(吕海江)$^{23}$, J.~G.~Lu(吕军光)$^{1,58}$, X.~L.~Lu(陆小玲)$^{1}$, Y.~Lu(卢宇)$^{7}$, Y.~P.~Lu(卢云鹏)$^{1,58}$, Z.~H.~Lu(卢泽辉)$^{1,64}$, C.~L.~Luo(罗成林)$^{41}$, J.~R.~Luo(罗家瑞)$^{59}$, M.~X.~Luo(罗民兴)$^{80}$, T.~Luo(罗涛)$^{12,g}$, X.~L.~Luo(罗小兰)$^{1,58}$, X.~R.~Lyu(吕晓睿)$^{64}$, Y.~F.~Lyu(吕翌丰)$^{43}$, F.~C.~Ma(马凤才)$^{40}$, H.~Ma(马衡)$^{79}$, H.~L.~Ma(马海龙)$^{1}$, J.~L.~Ma(马俊力)$^{1,64}$, L.~L.~Ma(马连良)$^{50}$, L.~R.~Ma(马立瑞)$^{67}$, M.~M.~Ma(马明明)$^{1,64}$, Q.~M.~Ma(马秋梅)$^{1}$, R.~Q.~Ma(马润秋)$^{1,64}$, T.~Ma(马腾)$^{72,58}$, X.~T.~Ma(马晓天)$^{1,64}$, X.~Y.~Ma(马骁妍)$^{1,58}$, Y.~M.~Ma(马玉明)$^{31}$, F.~E.~Maas$^{18}$, I.~MacKay$^{70}$, M.~Maggiora$^{75A,75C}$, S.~Malde$^{70}$, Y.~J.~Mao(冒亚军)$^{46,h}$, Z.~P.~Mao(毛泽普)$^{1}$, S.~Marcello$^{75A,75C}$, Z.~X.~Meng(孟召霞)$^{67}$, J.~G.~Messchendorp$^{13,65}$, G.~Mezzadri$^{29A}$, H.~Miao(妙晗)$^{1,64}$, T.~J.~Min(闵天觉)$^{42}$, R.~E.~Mitchell$^{27}$, X.~H.~Mo(莫晓虎)$^{1,58,64}$, B.~Moses$^{27}$, N.~Yu.~Muchnoi$^{4,c}$, J.~Muskalla$^{35}$, Y.~Nefedov$^{36}$, F.~Nerling$^{18,e}$, L.~S.~Nie(聂麟苏)$^{20}$, I.~B.~Nikolaev$^{4,c}$, Z.~Ning(宁哲)$^{1,58}$, S.~Nisar$^{11,m}$, Q.~L.~Niu(牛祺乐)$^{38,k,l}$, W.~D.~Niu(牛文迪)$^{55}$, Y.~Niu (牛艳)$^{50}$, S.~L.~Olsen$^{64}$, S.~L.~Olsen$^{10,64}$, Q.~Ouyang(欧阳群)$^{1,58,64}$, S.~Pacetti$^{28B,28C}$, X.~Pan(潘祥)$^{55}$, Y.~Pan(潘越)$^{57}$, A.~~Pathak$^{34}$, Y.~P.~Pei(裴宇鹏)$^{72,58}$, M.~Pelizaeus$^{3}$, H.~P.~Peng(彭海平)$^{72,58}$, Y.~Y.~Peng(彭云翊)$^{38,k,l}$, K.~Peters$^{13,e}$, J.~L.~Ping(平加伦)$^{41}$, R.~G.~Ping(平荣刚)$^{1,64}$, S.~Plura$^{35}$, V.~Prasad$^{33}$, F.~Z.~Qi(齐法制)$^{1}$, H.~Qi(齐航)$^{72,58}$, H.~R.~Qi(漆红荣)$^{61}$, M.~Qi(祁鸣)$^{42}$, T.~Y.~Qi(齐天钰)$^{12,g}$, S.~Qian(钱森)$^{1,58}$, W.~B.~Qian(钱文斌)$^{64}$, C.~F.~Qiao(乔从丰)$^{64}$, X.~K.~Qiao(乔晓珂)$^{81}$, J.~J.~Qin(秦佳佳)$^{73}$, L.~Q.~Qin(秦丽清)$^{14}$, L.~Y.~Qin(秦龙宇)$^{72,58}$, X.~P.~Qin(覃潇平)$^{12,g}$, X.~S.~Qin(秦小帅)$^{50}$, Z.~H.~Qin(秦中华)$^{1,58}$, J.~F.~Qiu(邱进发)$^{1}$, Z.~H.~Qu(屈子皓)$^{73}$, C.~F.~Redmer$^{35}$, K.~J.~Ren(任旷洁)$^{39}$, A.~Rivetti$^{75C}$, M.~Rolo$^{75C}$, G.~Rong(荣刚)$^{1,64}$, Ch.~Rosner$^{18}$, M.~Q.~Ruan(阮曼奇)$^{1,58}$, S.~N.~Ruan(阮氏宁)$^{43}$, N.~Salone$^{44}$, A.~Sarantsev$^{36,d}$, Y.~Schelhaas$^{35}$, K.~Schoenning$^{76}$, M.~Scodeggio$^{29A}$, K.~Y.~Shan(尚科羽)$^{12,g}$, W.~Shan(单葳)$^{24}$, X.~Y.~Shan(单心钰)$^{72,58}$, Z.~J.~Shang(尚子杰)$^{38,k,l}$, J.~F.~Shangguan(上官剑锋)$^{16}$, L.~G.~Shao(邵立港)$^{1,64}$, M.~Shao(邵明)$^{72,58}$, C.~P.~Shen(沈成平)$^{12,g}$, H.~F.~Shen(沈宏飞)$^{1,8}$, W.~H.~Shen(沈文涵)$^{64}$, X.~Y.~Shen(沈肖雁)$^{1,64}$, B.~A.~Shi(施伯安)$^{64}$, H.~Shi(史华)$^{72,58}$, H.~C.~Shi(石煌超)$^{72,58}$, J.~L.~Shi(石家磊)$^{12,g}$, J.~Y.~Shi(石京燕)$^{1}$, Q.~Q.~Shi(石勤强)$^{55}$, S.~Y.~Shi(史书宇)$^{73}$, X.~Shi(史欣)$^{1,58}$, J.~J.~Song(宋娇娇)$^{19}$, T.~Z.~Song(宋天资)$^{59}$, W.~M.~Song(宋维民)$^{34,1}$, Y. ~J.~Song(宋宇镜)$^{12,g}$, Y.~X.~Song(宋昀轩)$^{46,h,n}$, S.~Sosio$^{75A,75C}$, S.~Spataro$^{75A,75C}$, F.~Stieler$^{35}$, S.~S~Su(苏闪闪)$^{40}$, Y.~J.~Su(粟杨捷)$^{64}$, G.~B.~Sun(孙光豹)$^{77}$, G.~X.~Sun(孙功星)$^{1}$, H.~Sun(孙昊)$^{64}$, H.~K.~Sun(孙浩凯)$^{1}$, J.~F.~Sun(孙俊峰)$^{19}$, K.~Sun(孙开)$^{61}$, L.~Sun(孙亮)$^{77}$, S.~S.~Sun(孙胜森)$^{1,64}$, T.~Sun$^{51,f}$, W.~Y.~Sun(孙文玉)$^{34}$, Y.~Sun(孙源)$^{9}$, Y.~J.~Sun(孙勇杰)$^{72,58}$, Y.~Z.~Sun(孙永昭)$^{1}$, Z.~Q.~Sun(孙泽群)$^{1,64}$, Z.~T.~Sun(孙振田)$^{50}$, C.~J.~Tang(唐昌建)$^{54}$, G.~Y.~Tang(唐光毅)$^{1}$, J.~Tang(唐健)$^{59}$, M.~Tang(唐嘉骏)$^{72,58}$, Y.~A.~Tang(唐迎澳)$^{77}$, L.~Y.~Tao(陶璐燕)$^{73}$, Q.~T.~Tao(陶秋田)$^{25,i}$, M.~Tat$^{70}$, J.~X.~Teng(滕佳秀)$^{72,58}$, V.~Thoren$^{76}$, W.~H.~Tian(田文辉)$^{59}$, Y.~Tian(田野)$^{31,64}$, Z.~F.~Tian(田喆飞)$^{77}$, I.~Uman$^{62B}$, Y.~Wan(万宇)$^{55}$, S.~J.~Wang (王少杰)$^{50}$, B.~Wang(王斌)$^{1}$, B.~L.~Wang(王滨龙)$^{64}$, Bo~Wang(王博)$^{72,58}$, D.~Y.~Wang(王大勇)$^{46,h}$, F.~Wang(王菲)$^{73}$, H.~J.~Wang(王泓鉴)$^{38,k,l}$, J.~J.~Wang(王家驹)$^{77}$, J.~P.~Wang (王吉鹏)$^{50}$, K.~Wang(王科)$^{1,58}$, L.~L.~Wang(王亮亮)$^{1}$, M.~Wang(王萌)$^{50}$, N.~Y.~Wang(王南洋)$^{64}$, S.~Wang(王石)$^{38,k,l}$, S.~Wang(王顺)$^{12,g}$, T. ~Wang(王婷)$^{12,g}$, T.~J.~Wang(王腾蛟)$^{43}$, W. ~Wang(王维)$^{73}$, W.~Wang(王为)$^{59}$, W.~P.~Wang(王维平)$^{35,58,72,o}$, X.~Wang(王轩)$^{46,h}$, X.~F.~Wang(王雄飞)$^{38,k,l}$, X.~J.~Wang(王希俊)$^{39}$, X.~L.~Wang(王小龙)$^{12,g}$, X.~N.~Wang(王新南)$^{1}$, Y.~Wang(王亦)$^{61}$, Y.~D.~Wang(王雅迪)$^{45}$, Y.~F.~Wang(王贻芳)$^{1,58,64}$, Y.~L.~Wang(王艺龙)$^{19}$, Y.~N.~Wang(王亚男)$^{45}$, Y.~Q.~Wang(王雨晴)$^{1}$, Yaqian~Wang(王亚乾)$^{17}$, Yi~Wang(王义)$^{61}$, Z.~Wang(王铮)$^{1,58}$, Z.~L. ~Wang(王治浪)$^{73}$, Z.~Y.~Wang(王至勇)$^{1,64}$, Ziyi~Wang(王子一)$^{64}$, D.~H.~Wei(魏代会)$^{14}$, F.~Weidner$^{69}$, S.~P.~Wen(文硕频)$^{1}$, Y.~R.~Wen(温亚冉)$^{39}$, U.~Wiedner$^{3}$, G.~Wilkinson$^{70}$, M.~Wolke$^{76}$, L.~Wollenberg$^{3}$, C.~Wu(吴晨)$^{39}$, J.~F.~Wu(吴金飞)$^{1,8}$, L.~H.~Wu(伍灵慧)$^{1}$, L.~J.~Wu(吴连近)$^{1,64}$, X.~Wu(吴潇)$^{12,g}$, X.~H.~Wu(伍雄浩)$^{34}$, Y.~Wu(吴言)$^{72,58}$, Y.~H.~Wu(吴业昊)$^{55}$, Y.~J.~Wu(吴英杰)$^{31}$, Z.~Wu(吴智)$^{1,58}$, L.~Xia(夏磊)$^{72,58}$, X.~M.~Xian(咸秀梅)$^{39}$, B.~H.~Xiang(向本后)$^{1,64}$, T.~Xiang(相腾)$^{46,h}$, D.~Xiao(肖栋)$^{38,k,l}$, G.~Y.~Xiao(肖光延)$^{42}$, S.~Y.~Xiao(肖素玉)$^{1}$, Y. ~L.~Xiao(肖云龙)$^{12,g}$, Z.~J.~Xiao(肖振军)$^{41}$, C.~Xie(谢陈)$^{42}$, X.~H.~Xie(谢昕海)$^{46,h}$, Y.~Xie(谢勇 )$^{50}$, Y.~G.~Xie(谢宇广)$^{1,58}$, Y.~H.~Xie(谢跃红)$^{6}$, Z.~P.~Xie(谢智鹏)$^{72,58}$, T.~Y.~Xing(邢天宇)$^{1,64}$, C.~F.~Xu$^{1,64}$, C.~J.~Xu(许创杰)$^{59}$, G.~F.~Xu(许国发)$^{1}$, H.~Y.~Xu(许皓月)$^{67,2,p}$, M.~Xu(徐明)$^{72,58}$, Q.~J.~Xu(徐庆君)$^{16}$, Q.~N.~Xu$^{30}$, W.~Xu(许威)$^{1}$, W.~L.~Xu(徐万伦)$^{67}$, X.~P.~Xu(徐新平)$^{55}$, Y.~Xu(徐月)$^{40}$, Y.~C.~Xu(胥英超)$^{78}$, Z.~S.~Xu(许昭燊)$^{64}$, F.~Yan(严芳)$^{12,g}$, L.~Yan(严亮)$^{12,g}$, W.~B.~Yan(鄢文标)$^{72,58}$, W.~C.~Yan(闫文成)$^{81}$, X.~Q.~Yan(严薛强)$^{1,64}$, H.~J.~Yang(杨海军)$^{51,f}$, H.~L.~Yang(杨昊霖)$^{34}$, H.~X.~Yang(杨洪勋)$^{1}$, T.~Yang(杨涛)$^{1}$, Y.~Yang(杨莹)$^{12,g}$, Y.~F.~Yang(杨翊凡)$^{1,64}$, Y.~F.~Yang(杨艳芳)$^{43}$, Y.~X.~Yang(杨逸翔)$^{1,64}$, Z.~W.~Yang(杨政武)$^{38,k,l}$, Z.~P.~Yao(姚志鹏)$^{50}$, M.~Ye(叶梅)$^{1,58}$, M.~H.~Ye(叶铭汉)$^{8}$, J.~H.~Yin(殷俊昊)$^{1}$, Junhao~Yin(殷俊昊)$^{43}$, Z.~Y.~You(尤郑昀)$^{59}$, B.~X.~Yu(俞伯祥)$^{1,58,64}$, C.~X.~Yu(喻纯旭)$^{43}$, G.~Yu(余刚)$^{1,64}$, J.~S.~Yu(俞洁晟)$^{25,i}$, M.~C.~Yu$^{40}$, T.~Yu(于涛)$^{73}$, X.~D.~Yu(余旭东)$^{46,h}$, Y.~C.~Yu(于勇超)$^{81}$, C.~Z.~Yuan(苑长征)$^{1,64}$, J.~Yuan(袁菁)$^{34}$, J.~Yuan(袁杰)$^{45}$, L.~Yuan(袁丽)$^{2}$, S.~C.~Yuan(苑思成)$^{1,64}$, Y.~Yuan(袁野)$^{1,64}$, Z.~Y.~Yuan(袁朝阳)$^{59}$, C.~X.~Yue(岳崇兴)$^{39}$, A.~A.~Zafar$^{74}$, F.~R.~Zeng(曾凡蕊)$^{50}$, S.~H.~Zeng$^{63A,63B,63C,63D}$, X.~Zeng(曾鑫)$^{12,g}$, Y.~Zeng(曾云)$^{25,i}$, Y.~J.~Zeng(曾宇杰)$^{59}$, Y.~J.~Zeng(曾溢嘉)$^{1,64}$, X.~Y.~Zhai(翟星晔)$^{34}$, Y.~C.~Zhai(翟云聪)$^{50}$, Y.~H.~Zhan(詹永华)$^{59}$, A.~Q.~Zhang(张安庆)$^{1,64}$, B.~L.~Zhang(张伯伦)$^{1,64}$, B.~X.~Zhang(张丙新)$^{1}$, D.~H.~Zhang(张丹昊)$^{43}$, G.~Y.~Zhang(张广义)$^{19}$, H.~Zhang(张晗)$^{81}$, H.~Zhang(张豪)$^{72,58}$, H.~C.~Zhang(张航畅)$^{1,58,64}$, H.~H.~Zhang(张宏宏)$^{34}$, H.~H.~Zhang(张宏浩)$^{59}$, H.~Q.~Zhang(张华桥)$^{1,58,64}$, H.~R.~Zhang(张浩然)$^{72,58}$, H.~Y.~Zhang(章红宇)$^{1,58}$, J.~Zhang(张晋)$^{59}$, J.~Zhang(张进)$^{81}$, J.~J.~Zhang(张进军)$^{52}$, J.~L.~Zhang(张杰磊)$^{20}$, J.~Q.~Zhang(张敬庆)$^{41}$, J.~S.~Zhang(张家声)$^{12,g}$, J.~W.~Zhang(张家文)$^{1,58,64}$, J.~X.~Zhang(张景旭)$^{38,k,l}$, J.~Y.~Zhang(张建勇)$^{1}$, J.~Z.~Zhang(张景芝)$^{1,64}$, Jianyu~Zhang(张剑宇)$^{64}$, L.~M.~Zhang(张黎明)$^{61}$, Lei~Zhang(张雷)$^{42}$,
  N.~Zhang(张楠)$^{81}$,
  P.~Zhang(张鹏)$^{1,64}$, Q.~Y.~Zhang(张秋岩)$^{34}$, R.~Y.~Zhang(张若愚)$^{38,k,l}$, S.~H.~Zhang(张水涵)$^{1,64}$, Shulei~Zhang(张书磊)$^{25,i}$, X.~M.~Zhang(张晓梅)$^{1}$, X.~Y~Zhang$^{40}$, X.~Y.~Zhang(张学尧)$^{50}$, Y.~Zhang(张瑶)$^{1}$, Y. ~Zhang(张宇)$^{73}$, Y. ~T.~Zhang(张亚腾)$^{81}$, Y.~H.~Zhang(张银鸿)$^{1,58}$, Y.~M.~Zhang(张悦明)$^{39}$, Yan~Zhang(张言)$^{72,58}$, Z.~D.~Zhang(张正德)$^{1}$, Z.~H.~Zhang(张泽恒)$^{1}$, Z.~L.~Zhang(张兆领)$^{34}$, Z.~Y.~Zhang(张振宇)$^{77}$, Z.~Y.~Zhang(张子羽)$^{43}$, Z.~Z. ~Zhang(张子扬)$^{45}$, G.~Zhao(赵光)$^{1}$, J.~Y.~Zhao(赵静宜)$^{1,64}$, J.~Z.~Zhao(赵京周)$^{1,58}$, L.~Zhao(赵玲)$^{1}$, Lei~Zhao(赵雷)$^{72,58}$, M.~G.~Zhao(赵明刚)$^{43}$, N.~Zhao(赵宁)$^{79}$, R.~P.~Zhao(赵若平)$^{64}$, S.~J.~Zhao(赵书俊)$^{81}$, Y.~B.~Zhao(赵豫斌)$^{1,58}$, Y.~X.~Zhao(赵宇翔)$^{31,64}$, Z.~G.~Zhao(赵政国)$^{72,58}$, A.~Zhemchugov$^{36,b}$, B.~Zheng(郑波)$^{73}$, B.~M.~Zheng(郑变敏)$^{34}$, J.~P.~Zheng(郑建平)$^{1,58}$, W.~J.~Zheng(郑文静)$^{1,64}$, Y.~H.~Zheng(郑阳恒)$^{64}$, B.~Zhong(钟彬)$^{41}$, X.~Zhong(钟鑫)$^{59}$, H. ~Zhou( 周航)$^{50}$, J.~Y.~Zhou(周佳莹)$^{34}$, L.~P.~Zhou(周利鹏)$^{1,64}$, S. ~Zhou(周帅)$^{6}$, X.~Zhou(周详)$^{77}$, X.~K.~Zhou(周晓康)$^{6}$, X.~R.~Zhou(周小蓉)$^{72,58}$, X.~Y.~Zhou(周兴玉)$^{39}$, Y.~Z.~Zhou(周袆卓)$^{12,g}$, Z.~C.~Zhou(周章丞)$^{20}$, A.~N.~Zhu(朱傲男)$^{64}$, J.~Zhu(朱江)$^{43}$, K.~Zhu(朱凯)$^{1}$, K.~J.~Zhu(朱科军)$^{1,58,64}$, K.~S.~Zhu(朱康帅)$^{12,g}$, L.~Zhu(朱林)$^{34}$, L.~X.~Zhu(朱琳萱)$^{64}$, S.~H.~Zhu(朱世海)$^{71}$, T.~J.~Zhu(朱腾蛟)$^{12,g}$, W.~D.~Zhu(朱稳定)$^{41}$, Y.~C.~Zhu(朱莹春)$^{72,58}$, Z.~A.~Zhu(朱自安)$^{1,64}$, J.~H.~Zou(邹佳恒)$^{1}$, J.~Zu(祖健)$^{72,58}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{4}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{9}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{10}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{11}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{14}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{15}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{16}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{17}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{18}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{19}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{20}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{21}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{22}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{23}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{24}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{25}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{26}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{27}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{28}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{29}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{30}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{31}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{32}$ Institute of Physics and Technology, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{33}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{34}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{35}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{36}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{37}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{38}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{39}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{40}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{41}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{42}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{43}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{44}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{45}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{46}$ Peking University, Beijing 100871, People's Republic of China\\
$^{47}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{48}$ Renmin University of China, Beijing 100872, People's Republic of China\\
$^{49}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{50}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{51}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{52}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{53}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{54}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{55}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{56}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{57}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{58}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{59}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{60}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{61}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{62}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{63}$ University of Bristol, (A)H H Wills Physics Laboratory; (B)Tyndall Avenue; (C)Bristol; (D)BS8 1TL\\
$^{64}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{65}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{66}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{67}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{68}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{69}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{70}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{71}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{72}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{73}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{74}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{75}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{76}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{77}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{78}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{79}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{80}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{81}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Deceased\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{d}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{e}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{f}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{g}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{h}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{i}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{j}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{k}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at the Department of Mathematical Sciences, IBA, Karachi 75270, Pakistan\\
$^{n}$ Also at Ecole Polytechnique Federale de Lausanne (EPFL), CH-1015 Lausanne, Switzerland\\
$^{o}$ Also at Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{p}$ Also at School of Physics, Beihang University, Beijing 100191 , China\\
}}
%\end{center}

%\vspace{0.4cm}
%\end{small}


==> Source/name.tex <==
%\author{Author list}
\begin{small}
\begin{center}
M.~Ablikim$^{1}$, M.~N.~Achasov$^{4,c}$, P.~Adlarson$^{77}$, X.~C.~Ai$^{82}$, R.~Aliberti$^{36}$, A.~Amoroso$^{76A,76C}$, Q.~An$^{73,59,a}$, Y.~Bai$^{58}$, O.~Bakina$^{37}$, Y.~Ban$^{47,h}$, H.-R.~Bao$^{65}$, V.~Batozskaya$^{1,45}$, K.~Begzsuren$^{33}$, N.~Berger$^{36}$, M.~Berlowski$^{45}$, M.~Bertani$^{29A}$, D.~Bettoni$^{30A}$, F.~Bianchi$^{76A,76C}$, E.~Bianco$^{76A,76C}$, A.~Bortone$^{76A,76C}$, I.~Boyko$^{37}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{70}$, H.~Cai$^{78}$, M.~H.~Cai$^{39,k,l}$, X.~Cai$^{1,59}$, A.~Calcaterra$^{29A}$, G.~F.~Cao$^{1,65}$, N.~Cao$^{1,65}$, S.~A.~Cetin$^{63A}$, X.~Y.~Chai$^{47,h}$, J.~F.~Chang$^{1,59}$, G.~R.~Che$^{44}$, Y.~Z.~Che$^{1,59,65}$, C.~H.~Chen$^{9}$, Chao~Chen$^{56}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,65}$, H.~Y.~Chen$^{21}$, M.~L.~Chen$^{1,59,65}$, S.~J.~Chen$^{43}$, S.~L.~Chen$^{46}$, S.~M.~Chen$^{62}$, T.~Chen$^{1,65}$, X.~R.~Chen$^{32,65}$, X.~T.~Chen$^{1,65}$, X.~Y.~Chen$^{12,g}$, Y.~B.~Chen$^{1,59}$, Y.~Q.~Chen$^{35}$, Y.~Q.~Chen$^{16}$, Z.~J.~Chen$^{26,i}$, Z.~K.~Chen$^{60}$, S.~K.~Choi$^{10}$, X. ~Chu$^{12,g}$, G.~Cibinetto$^{30A}$, F.~Cossio$^{76C}$, J.~Cottee-Meldrum$^{64}$, J.~J.~Cui$^{51}$, H.~L.~Dai$^{1,59}$, J.~P.~Dai$^{80}$, A.~Dbeyssi$^{19}$, R.~ E.~de Boer$^{3}$, D.~Dedovich$^{37}$, C.~Q.~Deng$^{74}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{36}$, I.~Denysenko$^{37}$, M.~Destefanis$^{76A,76C}$, F.~De~Mori$^{76A,76C}$, B.~Ding$^{68,1}$, X.~X.~Ding$^{47,h}$, Y.~Ding$^{35}$, Y.~Ding$^{41}$, Y.~X.~Ding$^{31}$, J.~Dong$^{1,59}$, L.~Y.~Dong$^{1,65}$, M.~Y.~Dong$^{1,59,65}$, X.~Dong$^{78}$, M.~C.~Du$^{1}$, S.~X.~Du$^{82}$, S.~X.~Du$^{12,g}$, Y.~Y.~Duan$^{56}$, P.~Egorov$^{37,b}$, G.~F.~Fan$^{43}$, J.~J.~Fan$^{20}$, Y.~H.~Fan$^{46}$, J.~Fang$^{1,59}$, J.~Fang$^{60}$, S.~S.~Fang$^{1,65}$, W.~X.~Fang$^{1}$, Y.~Q.~Fang$^{1,59}$, R.~Farinelli$^{30A}$, L.~Fava$^{76B,76C}$, F.~Feldbauer$^{3}$, G.~Felici$^{29A}$, C.~Q.~Feng$^{73,59}$, J.~H.~Feng$^{16}$, L.~Feng$^{39,k,l}$, Q.~X.~Feng$^{39,k,l}$, Y.~T.~Feng$^{73,59}$, M.~Fritsch$^{3}$, C.~D.~Fu$^{1}$, J.~L.~Fu$^{65}$, Y.~W.~Fu$^{1,65}$, H.~Gao$^{65}$, X.~B.~Gao$^{42}$, Y.~Gao$^{73,59}$, Y.~N.~Gao$^{47,h}$, Y.~N.~Gao$^{20}$, Y.~Y.~Gao$^{31}$, S.~Garbolino$^{76C}$, I.~Garzia$^{30A,30B}$, P.~T.~Ge$^{20}$, Z.~W.~Ge$^{43}$, C.~Geng$^{60}$, E.~M.~Gersabeck$^{69}$, A.~Gilman$^{71}$, K.~Goetzen$^{13}$, J.~D.~Gong$^{35}$, L.~Gong$^{41}$, W.~X.~Gong$^{1,59}$, W.~Gradl$^{36}$, S.~Gramigna$^{30A,30B}$, M.~Greco$^{76A,76C}$, M.~H.~Gu$^{1,59}$, Y.~T.~Gu$^{15}$, C.~Y.~Guan$^{1,65}$, A.~Q.~Guo$^{32}$, L.~B.~Guo$^{42}$, M.~J.~Guo$^{51}$, R.~P.~Guo$^{50}$, Y.~P.~Guo$^{12,g}$, A.~Guskov$^{37,b}$, J.~Gutierrez$^{28}$, K.~L.~Han$^{65}$, T.~T.~Han$^{1}$, F.~Hanisch$^{3}$, K.~D.~Hao$^{73,59}$, X.~Q.~Hao$^{20}$, F.~A.~Harris$^{67}$, K.~K.~He$^{56}$, K.~L.~He$^{1,65}$, F.~H.~Heinsius$^{3}$, C.~H.~Heinz$^{36}$, Y.~K.~Heng$^{1,59,65}$, C.~Herold$^{61}$, P.~C.~Hong$^{35}$, G.~Y.~Hou$^{1,65}$, X.~T.~Hou$^{1,65}$, Y.~R.~Hou$^{65}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,65}$, J.~F.~Hu$^{57,j}$, Q.~P.~Hu$^{73,59}$, S.~L.~Hu$^{12,g}$, T.~Hu$^{1,59,65}$, Y.~Hu$^{1}$, Z.~M.~Hu$^{60}$, G.~S.~Huang$^{73,59}$, K.~X.~Huang$^{60}$, L.~Q.~Huang$^{32,65}$, P.~Huang$^{43}$, X.~T.~Huang$^{51}$, Y.~P.~Huang$^{1}$, Y.~S.~Huang$^{60}$, T.~Hussain$^{75}$, N.~H\"usken$^{36}$, N.~in der Wiesche$^{70}$, J.~Jackson$^{28}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{20}$, W.~Ji$^{1,65}$, X.~B.~Ji$^{1,65}$, X.~L.~Ji$^{1,59}$, Y.~Y.~Ji$^{51}$, Z.~K.~Jia$^{73,59}$, D.~Jiang$^{1,65}$, H.~B.~Jiang$^{78}$, P.~C.~Jiang$^{47,h}$, S.~J.~Jiang$^{9}$, T.~J.~Jiang$^{17}$, X.~S.~Jiang$^{1,59,65}$, Y.~Jiang$^{65}$, J.~B.~Jiao$^{51}$, J.~K.~Jiao$^{35}$, Z.~Jiao$^{24}$, S.~Jin$^{43}$, Y.~Jin$^{68}$, M.~Q.~Jing$^{1,65}$, X.~M.~Jing$^{65}$, T.~Johansson$^{77}$, S.~Kabana$^{34}$, N.~Kalantar-Nayestanaki$^{66}$, X.~L.~Kang$^{9}$, X.~S.~Kang$^{41}$, M.~Kavatsyuk$^{66}$, B.~C.~Ke$^{82}$, V.~Khachatryan$^{28}$, A.~Khoukaz$^{70}$, R.~Kiuchi$^{1}$, O.~B.~Kolcu$^{63A}$, B.~Kopf$^{3}$, M.~Kuessner$^{3}$, X.~Kui$^{1,65}$, N.~~Kumar$^{27}$, A.~Kupsc$^{45,77}$, W.~K\"uhn$^{38}$, Q.~Lan$^{74}$, W.~N.~Lan$^{20}$, T.~T.~Lei$^{73,59}$, M.~Lellmann$^{36}$, T.~Lenz$^{36}$, C.~Li$^{48}$, C.~Li$^{73,59}$, C.~Li$^{44}$, C.~H.~Li$^{40}$, C.~K.~Li$^{21}$, D.~M.~Li$^{82}$, F.~Li$^{1,59}$, G.~Li$^{1}$, H.~B.~Li$^{1,65}$, H.~J.~Li$^{20}$, H.~N.~Li$^{57,j}$, Hui~Li$^{44}$, J.~R.~Li$^{62}$, J.~S.~Li$^{60}$, K.~Li$^{1}$, K.~L.~Li$^{39,k,l}$, K.~L.~Li$^{20}$, L.~J.~Li$^{1,65}$, Lei~Li$^{49}$, M.~H.~Li$^{44}$, M.~R.~Li$^{1,65}$, P.~L.~Li$^{65}$, P.~R.~Li$^{39,k,l}$, Q.~M.~Li$^{1,65}$, Q.~X.~Li$^{51}$, R.~Li$^{18,32}$, S.~X.~Li$^{12}$, T. ~Li$^{51}$, T.~Y.~Li$^{44}$, W.~D.~Li$^{1,65}$, W.~G.~Li$^{1,a}$, X.~Li$^{1,65}$, X.~H.~Li$^{73,59}$, X.~L.~Li$^{51}$, X.~Y.~Li$^{1,8}$, X.~Z.~Li$^{60}$, Y.~Li$^{20}$, Y.~G.~Li$^{47,h}$, Y.~P.~Li$^{35}$, Z.~J.~Li$^{60}$, Z.~Y.~Li$^{80}$, H.~Liang$^{73,59}$, Y.~F.~Liang$^{55}$, Y.~T.~Liang$^{32,65}$, G.~R.~Liao$^{14}$, L.~B.~Liao$^{60}$, M.~H.~Liao$^{60}$, Y.~P.~Liao$^{1,65}$, J.~Libby$^{27}$, A. ~Limphirat$^{61}$, C.~C.~Lin$^{56}$, D.~X.~Lin$^{32,65}$, L.~Q.~Lin$^{40}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, B.~X.~Liu$^{78}$, C.~Liu$^{35}$, C.~X.~Liu$^{1}$, F.~Liu$^{1}$, F.~H.~Liu$^{54}$, Feng~Liu$^{6}$, G.~M.~Liu$^{57,j}$, H.~Liu$^{39,k,l}$, H.~B.~Liu$^{15}$, H.~H.~Liu$^{1}$, H.~M.~Liu$^{1,65}$, Huihui~Liu$^{22}$, J.~B.~Liu$^{73,59}$, J.~J.~Liu$^{21}$, K. ~Liu$^{74}$, K.~Liu$^{39,k,l}$, K.~Y.~Liu$^{41}$, Ke~Liu$^{23}$, L.~C.~Liu$^{44}$, Lu~Liu$^{44}$, M.~H.~Liu$^{12,g}$, P.~L.~Liu$^{1}$, Q.~Liu$^{65}$, S.~B.~Liu$^{73,59}$, T.~Liu$^{12,g}$, W.~K.~Liu$^{44}$, W.~M.~Liu$^{73,59}$, W.~T.~Liu$^{40}$, X.~Liu$^{39,k,l}$, X.~Liu$^{40}$, X.~K.~Liu$^{39,k,l}$, X.~Y.~Liu$^{78}$, Y.~Liu$^{82}$, Y.~Liu$^{82}$, Y.~Liu$^{39,k,l}$, Y.~B.~Liu$^{44}$, Z.~A.~Liu$^{1,59,65}$, Z.~D.~Liu$^{9}$, Z.~Q.~Liu$^{51}$, X.~C.~Lou$^{1,59,65}$, F.~X.~Lu$^{60}$, H.~J.~Lu$^{24}$, J.~G.~Lu$^{1,59}$, X.~L.~Lu$^{16}$, Y.~Lu$^{7}$, Y.~H.~Lu$^{1,65}$, Y.~P.~Lu$^{1,59}$, Z.~H.~Lu$^{1,65}$, C.~L.~Luo$^{42}$, J.~R.~Luo$^{60}$, J.~S.~Luo$^{1,65}$, M.~X.~Luo$^{81}$, T.~Luo$^{12,g}$, X.~L.~Luo$^{1,59}$, Z.~Y.~Lv$^{23}$, X.~R.~Lyu$^{65,p}$, Y.~F.~Lyu$^{44}$, Y.~H.~Lyu$^{82}$, F.~C.~Ma$^{41}$, H.~L.~Ma$^{1}$, J.~L.~Ma$^{1,65}$, L.~L.~Ma$^{51}$, L.~R.~Ma$^{68}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,65}$, R.~Y.~Ma$^{20}$, T.~Ma$^{73,59}$, X.~T.~Ma$^{1,65}$, X.~Y.~Ma$^{1,59}$, Y.~M.~Ma$^{32}$, F.~E.~Maas$^{19}$, I.~MacKay$^{71}$, M.~Maggiora$^{76A,76C}$, S.~Malde$^{71}$, Q.~A.~Malik$^{75}$, H.~X.~Mao$^{39,k,l}$, Y.~J.~Mao$^{47,h}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{76A,76C}$, A.~Marshall$^{64}$, F.~M.~Melendi$^{30A,30B}$, Y.~H.~Meng$^{65}$, Z.~X.~Meng$^{68}$, G.~Mezzadri$^{30A}$, H.~Miao$^{1,65}$, T.~J.~Min$^{43}$, R.~E.~Mitchell$^{28}$, X.~H.~Mo$^{1,59,65}$, B.~Moses$^{28}$, N.~Yu.~Muchnoi$^{4,c}$, J.~Muskalla$^{36}$, Y.~Nefedov$^{37}$, F.~Nerling$^{19,e}$, L.~S.~Nie$^{21}$, I.~B.~Nikolaev$^{4,c}$, Z.~Ning$^{1,59}$, S.~Nisar$^{11,m}$, Q.~L.~Niu$^{39,k,l}$, W.~D.~Niu$^{12,g}$, C.~Normand$^{64}$, S.~L.~Olsen$^{10,65}$, Q.~Ouyang$^{1,59,65}$, S.~Pacetti$^{29B,29C}$, X.~Pan$^{56}$, Y.~Pan$^{58}$, A.~Pathak$^{10}$, Y.~P.~Pei$^{73,59}$, M.~Pelizaeus$^{3}$, H.~P.~Peng$^{73,59}$, X.~J.~Peng$^{39,k,l}$, Y.~Y.~Peng$^{39,k,l}$, K.~Peters$^{13,e}$, K.~Petridis$^{64}$, J.~L.~Ping$^{42}$, R.~G.~Ping$^{1,65}$, S.~Plura$^{36}$, V.~Prasad$^{34}$, F.~Z.~Qi$^{1}$, H.~R.~Qi$^{62}$, M.~Qi$^{43}$, S.~Qian$^{1,59}$, W.~B.~Qian$^{65}$, C.~F.~Qiao$^{65}$, J.~H.~Qiao$^{20}$, J.~J.~Qin$^{74}$, J.~L.~Qin$^{56}$, L.~Q.~Qin$^{14}$, L.~Y.~Qin$^{73,59}$, P.~B.~Qin$^{74}$, X.~P.~Qin$^{12,g}$, X.~S.~Qin$^{51}$, Z.~H.~Qin$^{1,59}$, J.~F.~Qiu$^{1}$, Z.~H.~Qu$^{74}$, J.~Rademacker$^{64}$, C.~F.~Redmer$^{36}$, A.~Rivetti$^{76C}$, M.~Rolo$^{76C}$, G.~Rong$^{1,65}$, S.~S.~Rong$^{1,65}$, F.~Rosini$^{29B,29C}$, Ch.~Rosner$^{19}$, M.~Q.~Ruan$^{1,59}$, N.~Salone$^{45}$, A.~Sarantsev$^{37,d}$, Y.~Schelhaas$^{36}$, K.~Schoenning$^{77}$, M.~Scodeggio$^{30A}$, K.~Y.~Shan$^{12,g}$, W.~Shan$^{25}$, X.~Y.~Shan$^{73,59}$, Z.~J.~Shang$^{39,k,l}$, J.~F.~Shangguan$^{17}$, L.~G.~Shao$^{1,65}$, M.~Shao$^{73,59}$, C.~P.~Shen$^{12,g}$, H.~F.~Shen$^{1,8}$, W.~H.~Shen$^{65}$, X.~Y.~Shen$^{1,65}$, B.~A.~Shi$^{65}$, H.~Shi$^{73,59}$, J.~L.~Shi$^{12,g}$, J.~Y.~Shi$^{1}$, S.~Y.~Shi$^{74}$, X.~Shi$^{1,59}$, H.~L.~Song$^{73,59}$, J.~J.~Song$^{20}$, T.~Z.~Song$^{60}$, W.~M.~Song$^{35}$, Y. ~J.~Song$^{12,g}$, Y.~X.~Song$^{47,h,n}$, S.~Sosio$^{76A,76C}$, S.~Spataro$^{76A,76C}$, F.~Stieler$^{36}$, S.~S~Su$^{41}$, Y.~J.~Su$^{65}$, G.~B.~Sun$^{78}$, G.~X.~Sun$^{1}$, H.~Sun$^{65}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{20}$, K.~Sun$^{62}$, L.~Sun$^{78}$, S.~S.~Sun$^{1,65}$, T.~Sun$^{52,f}$, Y.~C.~Sun$^{78}$, Y.~H.~Sun$^{31}$, Y.~J.~Sun$^{73,59}$, Y.~Z.~Sun$^{1}$, Z.~Q.~Sun$^{1,65}$, Z.~T.~Sun$^{51}$, C.~J.~Tang$^{55}$, G.~Y.~Tang$^{1}$, J.~Tang$^{60}$, J.~J.~Tang$^{73,59}$, L.~F.~Tang$^{40}$, Y.~A.~Tang$^{78}$, L.~Y.~Tao$^{74}$, M.~Tat$^{71}$, J.~X.~Teng$^{73,59}$, J.~Y.~Tian$^{73,59}$, W.~H.~Tian$^{60}$, Y.~Tian$^{32}$, Z.~F.~Tian$^{78}$, I.~Uman$^{63B}$, B.~Wang$^{60}$, B.~Wang$^{1}$, Bo~Wang$^{73,59}$, C.~Wang$^{39,k,l}$, C.~~Wang$^{20}$, Cong~Wang$^{23}$, D.~Y.~Wang$^{47,h}$, H.~J.~Wang$^{39,k,l}$, J.~J.~Wang$^{78}$, K.~Wang$^{1,59}$, L.~L.~Wang$^{1}$, L.~W.~Wang$^{35}$, M.~Wang$^{51}$, M. ~Wang$^{73,59}$, N.~Y.~Wang$^{65}$, S.~Wang$^{12,g}$, T. ~Wang$^{12,g}$, T.~J.~Wang$^{44}$, W. ~Wang$^{74}$, W.~Wang$^{60}$, W.~P.~Wang$^{36,59,73,o}$, X.~Wang$^{47,h}$, X.~F.~Wang$^{39,k,l}$, X.~J.~Wang$^{40}$, X.~L.~Wang$^{12,g}$, X.~N.~Wang$^{1}$, Y.~Wang$^{62}$, Y.~D.~Wang$^{46}$, Y.~F.~Wang$^{1,59,65}$, Y.~H.~Wang$^{39,k,l}$, Y.~J.~Wang$^{73,59}$, Y.~L.~Wang$^{20}$, Y.~N.~Wang$^{78}$, Y.~Q.~Wang$^{1}$, Yaqian~Wang$^{18}$, Yi~Wang$^{62}$, Yuan~Wang$^{18,32}$, Z.~Wang$^{1,59}$, Z.~L. ~Wang$^{74}$, Z.~L.~Wang$^{2}$, Z.~Q.~Wang$^{12,g}$, Z.~Y.~Wang$^{1,65}$, D.~H.~Wei$^{14}$, H.~R.~Wei$^{44}$, F.~Weidner$^{70}$, S.~P.~Wen$^{1}$, Y.~R.~Wen$^{40}$, U.~Wiedner$^{3}$, G.~Wilkinson$^{71}$, M.~Wolke$^{77}$, C.~Wu$^{40}$, J.~F.~Wu$^{1,8}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{20}$, L.~J.~Wu$^{1,65}$, Lianjie~Wu$^{20}$, S.~G.~Wu$^{1,65}$, S.~M.~Wu$^{65}$, X.~Wu$^{12,g}$, X.~H.~Wu$^{35}$, Y.~J.~Wu$^{32}$, Z.~Wu$^{1,59}$, L.~Xia$^{73,59}$, X.~M.~Xian$^{40}$, B.~H.~Xiang$^{1,65}$, D.~Xiao$^{39,k,l}$, G.~Y.~Xiao$^{43}$, H.~Xiao$^{74}$, Y. ~L.~Xiao$^{12,g}$, Z.~J.~Xiao$^{42}$, C.~Xie$^{43}$, K.~J.~Xie$^{1,65}$, X.~H.~Xie$^{47,h}$, Y.~Xie$^{51}$, Y.~G.~Xie$^{1,59}$, Y.~H.~Xie$^{6}$, Z.~P.~Xie$^{73,59}$, T.~Y.~Xing$^{1,65}$, C.~F.~Xu$^{1,65}$, C.~J.~Xu$^{60}$, G.~F.~Xu$^{1}$, H.~Y.~Xu$^{2}$, H.~Y.~Xu$^{68,2}$, M.~Xu$^{73,59}$, Q.~J.~Xu$^{17}$, Q.~N.~Xu$^{31}$, T.~D.~Xu$^{74}$, W.~Xu$^{1}$, W.~L.~Xu$^{68}$, X.~P.~Xu$^{56}$, Y.~Xu$^{12,g}$, Y.~Xu$^{41}$, Y.~C.~Xu$^{79}$, Z.~S.~Xu$^{65}$, F.~Yan$^{12,g}$, H.~Y.~Yan$^{40}$, L.~Yan$^{12,g}$, W.~B.~Yan$^{73,59}$, W.~C.~Yan$^{82}$, W.~H.~Yan$^{6}$, W.~P.~Yan$^{20}$, X.~Q.~Yan$^{1,65}$, H.~J.~Yang$^{52,f}$, H.~L.~Yang$^{35}$, H.~X.~Yang$^{1}$, J.~H.~Yang$^{43}$, R.~J.~Yang$^{20}$, T.~Yang$^{1}$, Y.~Yang$^{12,g}$, Y.~F.~Yang$^{44}$, Y.~H.~Yang$^{43}$, Y.~Q.~Yang$^{9}$, Y.~X.~Yang$^{1,65}$, Y.~Z.~Yang$^{20}$, M.~Ye$^{1,59}$, M.~H.~Ye$^{8}$, Z.~J.~Ye$^{57,j}$, Junhao~Yin$^{44}$, Z.~Y.~You$^{60}$, B.~X.~Yu$^{1,59,65}$, C.~X.~Yu$^{44}$, G.~Yu$^{13}$, J.~S.~Yu$^{26,i}$, L.~Q.~Yu$^{12,g}$, M.~C.~Yu$^{41}$, T.~Yu$^{74}$, X.~D.~Yu$^{47,h}$, Y.~C.~Yu$^{82}$, C.~Z.~Yuan$^{1,65}$, H.~Yuan$^{1,65}$, J.~Yuan$^{46}$, J.~Yuan$^{35}$, L.~Yuan$^{2}$, S.~C.~Yuan$^{1,65}$, X.~Q.~Yuan$^{1}$, Y.~Yuan$^{1,65}$, Z.~Y.~Yuan$^{60}$, C.~X.~Yue$^{40}$, Ying~Yue$^{20}$, A.~A.~Zafar$^{75}$, S.~H.~Zeng$^{64A,64B,64C,64D}$, X.~Zeng$^{12,g}$, Y.~Zeng$^{26,i}$, Y.~J.~Zeng$^{60}$, Y.~J.~Zeng$^{1,65}$, X.~Y.~Zhai$^{35}$, Y.~H.~Zhan$^{60}$, A.~Q.~Zhang$^{1,65}$, B.~L.~Zhang$^{1,65}$, B.~X.~Zhang$^{1}$, D.~H.~Zhang$^{44}$, G.~Y.~Zhang$^{20}$, G.~Y.~Zhang$^{1,65}$, H.~Zhang$^{82}$, H.~Zhang$^{73,59}$, H.~C.~Zhang$^{1,59,65}$, H.~H.~Zhang$^{60}$, H.~Q.~Zhang$^{1,59,65}$, H.~R.~Zhang$^{73,59}$, H.~Y.~Zhang$^{1,59}$, J.~Zhang$^{82}$, J.~Zhang$^{60}$, J.~J.~Zhang$^{53}$, J.~L.~Zhang$^{21}$, J.~Q.~Zhang$^{42}$, J.~S.~Zhang$^{12,g}$, J.~W.~Zhang$^{1,59,65}$, J.~X.~Zhang$^{39,k,l}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,65}$, Jianyu~Zhang$^{65}$, L.~M.~Zhang$^{62}$, Lei~Zhang$^{43}$, N.~Zhang$^{82}$, P.~Zhang$^{1,8}$, Q.~Zhang$^{20}$, Q.~Y.~Zhang$^{35}$, R.~Y.~Zhang$^{39,k,l}$, S.~H.~Zhang$^{1,65}$, Shulei~Zhang$^{26,i}$, X.~M.~Zhang$^{1}$, X.~Y~Zhang$^{41}$, X.~Y.~Zhang$^{51}$, Y.~Zhang$^{1}$, Y. ~Zhang$^{74}$, Y. ~T.~Zhang$^{82}$, Y.~H.~Zhang$^{1,59}$, Y.~M.~Zhang$^{40}$, Y.~P.~Zhang$^{73,59}$, Z.~D.~Zhang$^{1}$, Z.~H.~Zhang$^{1}$, Z.~L.~Zhang$^{56}$, Z.~L.~Zhang$^{35}$, Z.~X.~Zhang$^{20}$, Z.~Y.~Zhang$^{44}$, Z.~Y.~Zhang$^{78}$, Z.~Z. ~Zhang$^{46}$, Zh.~Zh.~Zhang$^{20}$, G.~Zhao$^{1}$, J.~Y.~Zhao$^{1,65}$, J.~Z.~Zhao$^{1,59}$, L.~Zhao$^{1}$, L.~Zhao$^{73,59}$, M.~G.~Zhao$^{44}$, N.~Zhao$^{80}$, R.~P.~Zhao$^{65}$, S.~J.~Zhao$^{82}$, Y.~B.~Zhao$^{1,59}$, Y.~L.~Zhao$^{56}$, Y.~X.~Zhao$^{32,65}$, Z.~G.~Zhao$^{73,59}$, A.~Zhemchugov$^{37,b}$, B.~Zheng$^{74}$, B.~M.~Zheng$^{35}$, J.~P.~Zheng$^{1,59}$, W.~J.~Zheng$^{1,65}$, X.~R.~Zheng$^{20}$, Y.~H.~Zheng$^{65,p}$, B.~Zhong$^{42}$, C.~Zhong$^{20}$, H.~Zhou$^{36,51,o}$, J.~Q.~Zhou$^{35}$, J.~Y.~Zhou$^{35}$, S. ~Zhou$^{6}$, X.~Zhou$^{78}$, X.~K.~Zhou$^{6}$, X.~R.~Zhou$^{73,59}$, X.~Y.~Zhou$^{40}$, Y.~X.~Zhou$^{79}$, Y.~Z.~Zhou$^{12,g}$, A.~N.~Zhu$^{65}$, J.~Zhu$^{44}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,59,65}$, K.~S.~Zhu$^{12,g}$, L.~Zhu$^{35}$, L.~X.~Zhu$^{65}$, S.~H.~Zhu$^{72}$, T.~J.~Zhu$^{12,g}$, W.~D.~Zhu$^{42}$, W.~D.~Zhu$^{12,g}$, W.~J.~Zhu$^{1}$, W.~Z.~Zhu$^{20}$, Y.~C.~Zhu$^{73,59}$, Z.~A.~Zhu$^{1,65}$, X.~Y.~Zhuang$^{44}$, J.~H.~Zou$^{1}$, J.~Zu$^{73,59}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Bochum Ruhr-University, D-44780 Bochum, Germany\\
$^{4}$ Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{9}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{10}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{11}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{14}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{15}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{16}$ Guangxi University of Science and Technology, Liuzhou 545006, People's Republic of China\\
$^{17}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{18}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{19}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{20}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{21}$ Henan University, Kaifeng 475004, People's Republic of China\\
$^{22}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{23}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{24}$ Huangshan College, Huangshan 245000, People's Republic of China\\
$^{25}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{26}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{27}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{28}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{29}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{30}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara, I-44122, Ferrara, Italy\\
$^{31}$ Inner Mongolia University, Hohhot 010021, People's Republic of China\\
$^{32}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{33}$ Institute of Physics and Technology, Mongolian Academy of Sciences, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{34}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica 1000000, Chile\\
$^{35}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{36}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{37}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{38}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{39}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{40}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{41}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{42}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{43}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{44}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{45}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{46}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{47}$ Peking University, Beijing 100871, People's Republic of China\\
$^{48}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{49}$ Renmin University of China, Beijing 100872, People's Republic of China\\
$^{50}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{51}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{52}$ Shanghai Jiao Tong University, Shanghai 200240, People's Republic of China\\
$^{53}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{54}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{55}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{56}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{57}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{58}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{59}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{60}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{61}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{62}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{63}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{64}$ University of Bristol, H H Wills Physics Laboratory, Tyndall Avenue, Bristol, BS8 1TL, UK\\
$^{65}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{66}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{67}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{68}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{69}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{70}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{71}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{72}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{73}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{74}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{75}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{76}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{77}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{78}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{79}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{80}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{81}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{82}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Deceased\\
$^{b}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{c}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{d}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{e}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{f}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{g}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{h}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{i}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{j}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{k}$ Also at MOE Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{m}$ Also at the Department of Mathematical Sciences, IBA, Karachi 75270, Pakistan\\
$^{n}$ Also at Ecole Polytechnique Federale de Lausanne (EPFL), CH-1015 Lausanne, Switzerland\\
$^{o}$ Also at Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{p}$ Also at Hangzhou Institute for Advanced Study, University of Chinese Academy of Sciences, Hangzhou 310024, China\\
}\end{center}

\vspace{0.4cm}
\end{small}

==> acknowledgement_2024-04-24.tex <==
%% Saved at => 2023-08-29
\textbf{Acknowledgement}

Acknowledgement
The BESIII Collaboration thanks the staff of BEPCII and the IHEP computing center for their strong support. This work is supported in part by National Key R&D Program of China under Contracts Nos. 2020YFA0406300, 2020YFA0406400, 2023YFA1606000; National Natural Science Foundation of China (NSFC) under Contracts Nos. 11635010, 11735014, 11935015, 11935016, 11935018, 12025502, 12035009, 12035013, 12061131003, 12192260, 12192261, 12192262, 12192263, 12192264, 12192265, 12221005, 12225509, 12235017, 12361141819; the Chinese Academy of Sciences (CAS) Large-Scale Scientific Facility Program; the CAS Center for Excellence in Particle Physics (CCEPP); Joint Large-Scale Scientific Facility Funds of the NSFC and CAS under Contract No. U1832207; 100 Talents Program of CAS; The Institute of Nuclear and Particle Physics (INPAC) and Shanghai Key Laboratory for Particle Physics and Cosmology; German Research Foundation DFG under Contracts Nos. 455635585, FOR5327, GRK 2149; Istituto Nazionale di Fisica Nucleare, Italy; Ministry of Development of Turkey under Contract No. DPT2006K-120470; National Research Foundation of Korea under Contract No. NRF-2022R1A2C1092335; National Science and Technology fund of Mongolia; National Science Research and Innovation Fund (NSRF) via the Program Management Unit for Human Resources & Institutional Development, Research and Innovation of Thailand under Contracts Nos. B16F640076, B50G670107; Polish National Science Centre under Contract No. 2019/35/O/ST2/02907; The Swedish Research Council; U. S. Department of Energy under Contract No. DE-FG02-05ER41374
Other Fund Information
To be inserted with an additional sentence into papers that are relevant to the topic of special funding for specific topics. Authors can suggest which to Li Weiguo and/or the physics coordinator.
Example added sentence: This paper is also supported by the NSFC under Contract Nos. 10805053, 10979059, ....
National Natural Science Foundation of China (NSFC), 10805053, PWA
National Natural Science Foundation of China (NSFC), 10979059, Lund弦碎裂强子化模型及其通用强子产生器研究
National Natural Science Foundation of China (NSFC), 10775075,
National Natural Science Foundation of China (NSFC), 10979012, baryons
National Natural Science Foundation of China (NSFC), 10979038, charmonium
National Natural Science Foundation of China (NSFC), 10905034, psi(2S)->B Bbar
National Natural Science Foundation of China (NSFC), 10975093, D 介子
National Natural Science Foundation of China (NSFC), 10979033, psi(2S)->VP
National Natural Science Foundation of China (NSFC), 10979058, hc
National Natural Science Foundation of China (NSFC), 10975143, charmonium rare decays

